LiftTiles: Constructive Building Blocks for Prototyping Room-scale Shape-changing Interfaces

Large-scale shape-changing interfaces have great potential, but creating such systems requires substantial time, cost, space, and efforts, which hinders the research community to explore interactions beyond the scale of human hands. We introduce modular inflatable actuators as building blocks for prototyping room-scale shape-changing interfaces. Each actuator can change its height from 15cm to 150cm, actuated and controlled by air pressure. Each unit is low-cost (8 USD), lightweight (10 kg), compact (15 cm), and robust, making it well-suited for prototyping room-scale shape transformations. Moreover, our modular and reconfigurable design allows researchers and designers to quickly construct different geometries and to explore various applications. This paper contributes to the design and implementation of highly extendable inflatable actuators, and demonstrates a range of scenarios that can leverage this modular building block.

==> TEI 2020 - LiftTiles_ Constructive Building Blocks for Prototyping Room-scale Shape-changing Interfaces/0-abstract.tex <==

\begin{abstract}
Large-scale shape-changing interfaces have great potential, but creating such systems requires substantial time, cost, space, and efforts, which hinders the research community to explore interactions beyond the scale of human hands. We introduce modular inflatable actuators as building blocks for prototyping {\it room-scale} shape-changing interfaces.  Each actuator can change its height from 15cm to 150cm, actuated and controlled by air pressure. Each unit is low-cost (8 USD), lightweight (10 kg), compact (15 cm), and robust, making it well-suited for prototyping room-scale shape transformations. Moreover, our modular and reconfigurable design allows researchers and designers to quickly construct different geometries and to explore various applications. This paper contributes to the design and implementation of highly extendable inflatable actuators, and demonstrates a range of scenarios that can leverage this modular building block.
\end{abstract}

\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003120.10003121</concept_id>
<concept_desc>Human-centered computing~Human computer interaction (HCI)</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Human computer interaction (HCI)}
\keywords{inflatables, shape-changing interfaces, large-scale interactions}


% This paper proposes constructive building blocks for prototyping room-scale shape-changing interfaces.
% due to the technical challenges in scalability, robustness, and deployability.
% of reconfigurable room-scale shape-changing interfaces and discuss how this prototype environment can open up the new opportunity, 

% and light (e.g., 1.8kg), while extending up to 1.5m to allow for large-scale shape transformation. Inflatable actuation also provides a robust structure that can support heavy objects. Due to its modular design, users can easily deploy and rearrange Dynaroom units for different applications. This paper describes the design and implementation of Dynaroom and explores the application space 
% Dynaroom consists of an array of retractable and inflatable actuator that is compact (e.g., 15cm tall) and light (e.g., 1.8kg), while extending up to 1.5m to allow for large-scale shape transformation. Inflatable actuation also provides a robust structure  This paper describes the design and implementation of Dynaroom and explores the application space for reconfigurable room-scale shape displays. 
% a modular and reconfigurable room-scale shape display. Shape displays have been a promising approach to general-purpose shape-changing interfaces. However, most of the existing pin-based shape displays focus on interactions at the scale of a human hand, and due to , few explore larger-scale shape transformations. To overcome these challenges, this paper proposes 


==> TEI 2020 - LiftTiles_ Constructive Building Blocks for Prototyping Room-scale Shape-changing Interfaces/1-introduction.tex <==
\section{Introduction}
Emerging shape-changing user interfaces have great potential to transform interactions between humans and computers. 
In contrast to traditional graphical user interfaces, shape-changing interfaces provide rich physical affordances and haptic sensations by adapting their shape to the users' needs and context.
While prior work mostly focuses on shape-change of hand-held objects (e.g. shape-changing mobile phones~\cite{gomes2013morephone, nakagaki2015lineform, roudaut2013morphees, yao2013pneui}) or tabletop surfaces (e.g., shape displays~\cite{follmer2013inForm, iwata2001project, poupyrev2004lumen}), larger-scale shape transformation that engages the whole body has been proposed~\cite{green2016architectural, sturdee2015public}.
However, to construct and deploy such large-scale shape-changing interfaces requires substantial time and effort, at often prohibitive cost. These barriers restrict the research community to prototype and explore applications beyond the scale of the human hand. Our work is addressing this challenge by developing more accessible prototyping tools to help researchers, designers, and practitioners to explore the broader space of possible applications.

This paper introduces \tool{}, modular inflatable actuators for prototyping room-scale shape-changing interfaces.
Each inflatable actuator has a large footprint (e.g., 30 cm x 30 cm) and enables large-scale shape transformation.
The actuator is fabricated from a flexible plastic tube and constant force springs. It extends when inflated and retracts by the force of its spring when deflated. By controlling the internal air volume, the actuator can change its height from 15 cm to 150 cm (Figure~\ref{fig:cover} A-C).
We designed each module as low cost (e.g., 8 USD), lightweight (e.g., 1.8kg), and robust (e.g., withstand more than 10 kg weight), so that it is suitable for rapid prototyping of room-sized interfaces.
Inspired by reel-based pneumatic actuators~\cite{hammond2017pneumatic}, our design utilizes constant force springs to provide greater scalability, simplified fabrication, and stronger retraction force, all essential for large-scale shape-change. 
\changes{Building on our prior initial exploration of an inflatable actuator~\cite{suzuki2019lifttiles}, we describe the design rationale, technical details and limitations of our system in detail.}

\tool{} leverages modular and reconfigurable hardware building blocks. Designers can rearrange these blocks into various geometries to quickly explore different form factors and applications.
We demonstrate some prototyping example applications, such as a shape-changing floor for adaptive furniture, a shape-changing wall for dynamic partition and information display, and environmental haptic interfaces for immersive VR experiences.

This paper contributes:
\begin{enumerate}
% \item \tool{}, a proof-of-concept prototype for modular and reconfigurable room-scale shape displays.
\item Concept of a modular inflatable actuator as a building block for prototyping room-scale shape-changing interfaces.
\item Design and implementation of a highly extendable linear actuator that is low-cost, lightweight, compact, robust, and easy-to-fabricate.
\item A range of applications that demonstrate the potential of the system for prototyping room-scale shape transformation. 
\end{enumerate}


% An expert review with two architects and one interior designer reveals potential benefits and limitations and identifies the current \tool{} prototype.
% Based on this input, we demonstrate possible application scenarios, including public information displays, data physicalization, dynamic furniture, adaptive space separation, and room-scale haptics for virtual or augmented reality. 
% Their insights provide guidelines for the design of room-scale shape displays and direct the HCI community to further explore interactions with large-scale shape-changing interfaces.

% The actuators can share the air pump, so that quickly build different geometries by aligning them in both vertical (e.g. Figure~\cite{cover} D-F) and horizontal directions.


% a tool to prototype large-scale shape-changing interfaces and 
 % (e.g., interfaces at the scale of furniture, vehicle, room, building, and landscape).
% \item Expert review with three professionals to reveal the potential benefits and limitations of the current approach.
% Design and implementation of a retractable inflatable actuator that is compact, lightweight, robust, and highly extendable for room-scale shape changes.


% This enables a large actuator that expands from 15cm to 150cm, at a footprint of 30cm x 30cm.
% which we call deployable shape-changing blocks. To achieve this goal, we leverage a deployable inflatable structure.

% most of existing shape-changing interfaces focus on interactions at the scale of human hands, large-scale interactions are less explored.
% However, most of the existing systems often focus on the scale of human hands. When we try to scale them to a larger size, we face a lot of challenges, such as cost, deployability, and robustness of mechanical actuators. Due to this, most of such systems are only seen in large-scale installation, but it requires substantial cost, time, and space to deploy. Moreover, these installations are not suitable for customize, once built. For the research community, however, there are no casual and improvisational ways to design and explore how people can interact with shape-changing interfaces at large scale.

% It is promising to adapt to our needs and environment to provide rich affordances, haptics, and tactile sensation.
% These interfaces can be embedded in our environments, and make them responsive.
% It points to a path to make shape-changing interfaces more ubiquitous. 
% Due to the technical challenges, these interfaces can only be seen as a large-scale installation, 


% are often hypothetical 
% It lacks the 
% augment our static physical environment into a dynamic one. 


% \begin{figure}[!h]
% \centering
% \includegraphics[width=3.4in]{anonymous-figure/system-extend.png}
% \caption{A retractable inflatable actuator can extend from 15cm (A) to 150cm (C).}
% ~\label{fig:system-extend}
% \vspace{-0.6cm}
% \end{figure}

% Utilizing the \tool{} prototype system, we explore possible interactions with reconfigurable room-scale shape displays and propose three high-level interaction spaces: 1) {\it Adaption} to the user's needs and situation, 2) {\it Display} of information or data to the user, and 3) {\it Haptics} to provide physical feedback synchronized with visual information.


==> TEI 2020 - LiftTiles_ Constructive Building Blocks for Prototyping Room-scale Shape-changing Interfaces/2-related-work.tex <==
\section{Related Work}

\subsection{Inflatable Shape-Changing Interfaces}
Inflatables have long been a popular method for constructing large and lightweight architectural structures and artistic sculptures~\cite{farm1970inflatocookbook, piene2008sky}. 
These objects are usually passive after inflation, but HCI researchers have explored their use for dynamic shape-changing interfaces (e.g PneUI~\cite{yao2013pneui}, aeroMorph~\cite{ou2016aeroMorph}, JamSheets~\cite{ou2014jamsheets}, Printflatables~\cite{sareen2017printflatables}) and active haptic interfaces (e.g., ForceJacket~\cite{delazio2018force}, PuPoP~\cite{teng2018pupop}). 
\changes{Swaminathan et al. also explored room-scale deployable structures with inter-connected pneumatic trusses~\cite{swaminathan2019input}}
One key advantage of inflatables is their ability to transform their size and shape drastically. 
For example, reel-based pneumatic actuators~\cite{hammond2017pneumatic, hawkes2017soft} are highly extendable actuators for soft robots and shape-changing interfaces.
Our key technical contribution is to extend this line of work to a larger footprint (e.g., 30 cm x 30 cm) and enable a more robust structure (e.g., withstand 10 kg weight).
\changes{Most closely related to our work, TilePoP~\cite{teng2019tilepop} introduces a room-scale inflatable shape display for haptics in VR. Compared to the TilePop modules, our actuator employs a constant force spring for continuous, rather than discrete extension. The spring also removes the need for a vacuum pump, as it pushes out air when deflating. We also explore applications besides VR that leverage the general-purpose nature of modular, reconfigurable actuation blocks.}

\subsection{Prototyping Shape-changing Interfaces}
Shape-changing interfaces are technically challenging to build and control. Therefore, creating appropriate prototyping tools for these interfaces is considered one of the most important and critical goals in shape-changing UI research~\cite{alexander2018grand}.
Paper sketches are commonly used to design shape-changing interfaces~\cite{Rasmussen2016SketchingShapeChanging}, but they are static and lack the affordances of physical objects. Tools like ShapeClips~\cite{hardy2015shapeclip} and Kinetic Sketchup~\cite{Parkes2009Sketchup} have demonstrated how rapid physical prototyping tools enable designers to explore a range of applications in hours, rather than weeks.
\changes{For large-scale shape transformation, TrussFormer~\cite{kovacs2018trussformer} introduces a tool to design and prototype a large-scale kinetic transformation by actuating a static truss structure~\cite{kovacs2017trussfab}.
Prototyping tools for large-scale shape transformation could open up exciting application spaces~\cite{sturdee2015public}, but researchers still lack access to such tools. Our work contributes to this by introducing inexpensive, deployable and reconfigurable building blocks to rapidly prototype large-scale, functional shape-changing interfaces. We also propose example applications built with these building blocks.}
% These tools have demonstrated interactions at the scale of human hands.


\subsection{Large-scale Shape-changing Interfaces}
In the past, large-scale shape-change has been explored primarily in architecture and art.
For example, several large-scale ceiling-mounted or wall-based shape displays have been built (e.g., Kinetic sculpture at the BMW Museum~\cite{fermoso2008kinetic}, Breaking the Surface~\cite{rhodes_2014}, Hyposurface~\cite{goulthorpe2001aegis}, MegaFaces~\cite{khan2014megafaces}).
However, building these large installations requires tremendous time, cost, and efforts.
They are usually designed for a single-purpose installation and difficult to customize, once built.
In contrast, our goal is to provide a reconfigurable kit that supports rapid prototyping.
Some works explore a modular approach to construct dynamic furniture (e.g., Lift-bit~\cite{morillo2013radical}, Tangible Pixels~\cite{tang2011tangible}), but these electro-mechanical modules are expensive when a larger size and stronger force are required, placing them outside the reach of most researchers.
We aim to reduce the required cost and time by one or two orders of magnitude by leveraging low-cost and easy-to-fabricate inflatable actuation methods.
% To this end, we explore different design and fabrication to leverage inflatable deployable structure for constructive building blocks of prototyping room-scale shape-changing interfaces.







% and constructive shape displays for room-scale interactions. 
% This is mainly because of the cost and robustness of electro-mechanical actuators. We overcome these limitations by introducing retractable inflatable actuators with a compact, lightweight, and robust mechanism for room-scale shape changes.

% For example, the Muscle Tower~\cite{oosterhuis2008interactions} is a tall, open structural tower that leans and bends toward passers-by.
% Open Columns~\cite{khan2010open} and ExoBuilding~\cite{schnadelbach2010exobuilding} are ceiling-mounted actuators that respond and provide ambient physical data representations. 
% Gronvall et al.~\cite{gronvall2014causing} proposed a shape-changing bench and observed how users react with it in public space.
% However, these prior works are single-purpose concept demonstrations and are ill-suited to investigate the larger design space of interaction.




% Shape displays are a class of shape-changing interfaces that can render a 2.5D shape on a dynamic surface.
% By leveraging individually controlled linear actuator, previous works have demonstrated the ranges of applications (e.g., FEELEX~\cite{iwata2001project}, Lumen~\cite{poupyrev2004lumen}, inFORM~\cite{follmer2013inForm}).

% Previous work have greatly expanded this domain through exploring
% Recent work has expanded these methods for large-scale fabrication and interaction, e.g.  investigated fabrication techniques for body-scale shape-changing interfaces, 
% Inspired by these works and the potential for using pneumatics for actuation, we designed and prototyped a modular and scalable inflatable actuator for room-size shape displays.


% \subsection{Responsive Architecture}
% The twentieth century architect Le Corbusier famously referred to a house as a ``machine for living in'' and responsive architecture, buildings that can dynamically transform their physical structures, have attracted architects for decades, for example the whimsical work of Archigram~\cite{cook1999archigram}.
% Prominent examples include Hoberman's expandable architecture~\cite{antonelli2008design}, Jean Nouvel's kinetic facades~\cite[p.~19]{moloney2011designing}, and Tatlin's proposal for a helical tower with rotating structures~\cite{gorczyca2013motion}.
% Responsive architecture as a research area has only recently begun to receive serious attention in the HCI community ~\cite{gross2012architectural, takeuchi2014towards}.
% % add Squama by Jun Rekimoto

% Previous work has explored responsive spatial environments. 
% For example, the Muscle Tower~\cite{oosterhuis2008interactions} is a tall, open structural tower that leans and bends toward passers-by.
% Open Columns~\cite{khan2010open} and ExoBuilding~\cite{schnadelbach2010exobuilding} are ceiling-mounted actuators that respond and provide ambient physical data representations. 
% Gronvall et al.~\cite{gronvall2014causing} proposed a shape-changing bench and observed how users react with it in public space.
% However, these prior works are single-purpose concept demonstrations and are ill-suited to investigate the larger design space of interaction.
% In contrast to rapidly changing dynamic actuated building components, considering buildings on a much longer time scale (i.e., months and years rather than minutes and hours), N. John Habraken~\cite{habraken2000structure} developed design and construction methods to accommodate changing uses of a dwelling, and allow flexible and variable configurations.  In a similar vein, Stewart Brand~\cite{brand1995buildings} shows how reconfigurable elements enable adaptive and general-purpose structures that inhabitants can adapt to their changing needs. Inspired by this principle, we explore how modularity and reconfigurability can expand the interaction space of room-scale shape displays.



% Prior work also investigated interaction techniques using shape displays, such as gestural and direct manipulation~\cite{leithinger2011recompose, leithinger2011direct}, and various techniques to interact with physical data representations~\cite{taher2015exploring}.
% However, most of these works focus on interactions at the scale of a human hand, while room-scale transformations have been less examined. This opens an opportunity to explore new architectural applications~\cite{gross2012architectural, sturdee2015public}.

% However, the focus of these works is usually artistic and does not explore a wide range of user interactions and scenarios.

% Another problem of these large-scale shape displays is their difficulty of deployment.
% ShapeClip~\cite{hardy2015shapeclip} proposed a modular prototyping design for table-top shape displays, but larger shape displays still lack an appropriate design;
% most existing ceiling- and wall-based shape displays have a monolithic design, which significantly increases the cost of exploring interaction techniques.
% Thus, we apply the concept of modular shape displays proposed in \cite{hardy2015shapeclip} for prototyping  room-scale shape-changing interfaces.
% Similar to our work, Lift-bit~\cite{morillo2013radical} and Tangible Pixels~\cite{tang2011tangible} introduce a modular shape-changing unit based on electro-mechanical actuators.
% However, these designs have a limited extension ratio (less than x2), which restricts their range of transformation. This also means that the actuators require substantial space.




% a modular design for quick prototype and design exploration of such displays.
% Particularly for larger-scale shape displays, this has been an obstacle or HCI community to fabricate, deploy, and explore possible interactions.
% For larger-scale design, 
% While conceptually similar, these designs have limited extension ratio 

% and most of them have limited capability for user interaction, and less explored the possible interactions.
% Also, none of these works have provided the systematic considerations from the viewpoint of the technical and interaction perspectives.
% Thus, this paper contributes to discuss the technical trade-offs between different actuation mechanisms, and explore untapped interaction space enabled by a pin-based large-scale shape 
% % Thus, this paper investigates the 



% refers to a class of architectures which can provide dynamic tangible outputs using kinetic transformation.
% These concepts have attracted architects for a long time.
% building dynamics which allows the inhabitants changing 
% through a simple and easily reconfigurable elements can 
% The Related work is adequate, but I would like to take the opportunity to point the authors to the book ‘How Buildings Learn: What Happens After They’re Built’ if they are not a prior familiar with that book. I think it can provide some interesting aspects of building dynamics and how buildings change over time due to the inhabitants changing and emerging needs.
% We anticipate a simple, low-cost, and easily reconfigurable modular elements are key for adaptive and general-purpose structures. 
% Thus, this work 

% Dress Room~\cite{vallgaarda2014dress} responds to the location/position of an inhabitant, measured through pressure sensors integrated into the floor.
% variations in carbon-dioxide levels in interior spaces or the user's physiological data.
% These works are designed to map data into architectural space as an ambient but physical data representation. 



% For shape-changing interfaces, large-scale shape-changing capability is one of the most interesting domains. 
% For example, the public ideation of shape-changing interfaces~\cite{sturdee2015public} has also identified large-scale shape-changing as one of the most promising applications for shape-changing interfaces.
% Gronvall et al.~\cite{gronvall2014causing} have studies how the users react with the shape-changing bench through observing the public space.
% It is still not clear 
% But these ideas have primarily been explored in an artistic and design context.




% Although these works have investigated the design space of pneumatic actuation, the demonstration focuses on small scale shape-change.
% It also continues a tradition of deploying inflatable structures in architecture, pioneered by the \emph{Inflatocookbook}~\cite{farm1970inflatocookbook}.
% Inspired from the soft robotic literature, recent HCI research has demonstrated these principles for soft material interfaces. 


%  which can extend up to twice as its initial height.
% These are conceptually similar, but previous work has not fully investigated the tradeoffs between cost and scalability.
% Also, its design only allows the low extension ratio up to two times, thus it requires substantial space for the mechanical actuators, which introduces difficulties in installation and limits the capability of shape changes.
% In contrast, we proposes a pneumatic linear actuator as a scalable and highly extendable low-cost actuation that can extend up to ten times, and introduce two different types of shape displays, leveraging this form factor.

% rendering dynamic material properties~\cite{nakagaki2016materiable}.
% To interact with a shape display, prior work investigates the gestural and direct manipulation 
% While the rendered shapes is limited to 2.5D shapes, recent work has explored ways to address this limitation by assembling blocks to create graspable 3D shape.
% explored the shape display for dynamic data representation~\cite{taher2015exploring}.


% Since a common problem of shape displays is its large and monolithic design and high fabrication cost, 
% In recent years, these interfaces can 
% shapeShift have explored haptic interfaces for virtual reality \cite{siu2018shapeShift}.
% In the previous work, researchers have also investigated the use of shape displays for a range of user interactions, such as the haptic feedback for graphical information and to render dynamic physical affordances x, support gestural and direct manipulation . 
% Shape displays are one of the promising approaches for general-purpose shape-changing interfaces.


% Taking inspiration from this work, we anticipate the modular approach
% We anticipate the pin-based shape display would be more suitable for user interactions, as it allows more interaction capabilities. 
% As we mentioned in the introduction, there are several technical challenges to scale up to the shape displays.
% While there are relatively few, some prior work investigates the large-scale shape displays. 
% But these ideas have primarily been explored in an artistic and design context.
% Outside of the 
% For more general-purpose shape-changing, there are a number of prior works exploring ceiling-based shape displays~\cite{sauter2014sensitive}.
% For example, BMW Museum, Breaking the Surface is a ceiling-based shape display which can react to people walking underneath \cite{rhodes_2014}.
% Alternatively, there are some wall-based shape displays 
% However, the primary focus of these displays is on artistic rendering and installation, less focusing on interaction.


% In contrast to the other ceiling or wall-based shape displays, the pin-based displays have a great potential for applications in user interaction. 









% While there is relatively less work in large-scale shape-changing interfaces, previous work have investigated the potential use scenario of the large-scale shape changing.
% This may be aided by the recent fascination with HCI with shapeshifting user interfaces, which can potentially yield new technologies applicable to the design of such structures.
% and some examples can be seen in revolving restaurants, retractable stadium roofs, and media facades
% As such factors are critical for actual deployment, 



% relatively few works in larger-scale shape-changing interfaces, previous work have investigated user interaction with shape-changing furniture.
% These include the dynamic affordances, remote collaborations, data visualization, providing haptics and tactile sensations, and accessibility assistant. 


% room- and architecture-scale.
% Recent technological advances in shape changing interfaces promise to augment the current dynamic architecture. 

% However, there is less work on wall- or floor-based shape displays, although these configurations are interesting from the interaction perspective as the user can directly touch, sit, and lie on a display.
% A major reason of the scalability issue stems from the underlying technology: while several different actuation mechanisms have been proposed, most inexpensive mechanical actuators are not suitable for the actuation of large and heavy objects. To overcome these issues, we design and develop a custom pneumatic actuator, which enables the low-cost and scalable fabrication of large-scale shape displays. 

% While there are relatively few works in larger-scale shape-changing interfaces, previous work have investigated user interaction with shape-changing furniture.
% For example, Gronvall et al.~\cite{gronvall2014causing} have studies how the users react with the shape-changing bench through observing the public space. The public ideation of shape-changing interfaces~\cite{sturdee2015public} has also identified large-scale shape-changing as one of the most promising applications for shape-changing interfaces. 
% %They studied and zdiscussed what kind of interactions can be possible through public ideation, and it provide several interesting ideas.
% %However, these work lack a serious consideration about how to achieve from the technical perspective. 


==> TEI 2020 - LiftTiles_ Constructive Building Blocks for Prototyping Room-scale Shape-changing Interfaces/3-system.tex <==
\section{LiftTiles: System Design}

\subsection{Overview}

This section describes the design and implementation of our modular inflatable actuator and how we use it to construct room-scale shape-changing interfaces.

\begin{figure}[!h]
\centering
\includegraphics[width=3.2in]{final-figures/system-mechanism.pdf}
\caption{Mechanism of our inflatable actuator.}
~\label{fig:system-mechanism}
\vspace{-0.6cm}
\end{figure}

Our inflatable actuator leverages an extendable structure similar to a party horn.
Each inflatable actuator consists of a flexible plastic tube and two constant force springs, which are rolled at their resting positions (Figure~\ref{fig:system-mechanism}).
When pumping air into the tube, the actuator extends as the internal air pressure increases and the end of the tube unwinds. When releasing air through a release valve, the inflatable tube retracts due to the force of the embedded spring returning to its resting position.

\begin{figure}[!h]
\centering
% \includegraphics[width=3.4in]{final-figures/system-cad-illust.jpg}
% \hspace{0.02in}
\includegraphics[width=1.5in]{final-figures/system-cad-illust-1.pdf}
\hspace{0.04in}
\includegraphics[width=1.65in]{final-figures/system-cad-illust-2.jpg}
\caption{Each actuator consists of a plastic tube and constant force springs, which extend from 15 cm to 150cm when inflated and retract when deflated.}
~\label{fig:mechanical-design}
% \vspace{-0.3cm}
\end{figure}

Figure~\ref{fig:mechanical-design} and~\ref{fig:system-cad} illustrates an overview of our actuator design.
Our design is inspired by the prior reel-based actuator~\cite{agrawal2015protopiper, hammond2017pneumatic, hawkes2017soft, suzuki2019shapebots, takei2011kinereels}, which enables the highly extendable structure.
Particularly, Hammond et al.~\cite{hammond2017pneumatic} pioneered the highly extendable reel-based actuator with pneumatic actuation. However, as we built prototypes, we realized that the force of the spiral torsion springs and the 3D printed enclosure used in \cite{hammond2017pneumatic} were too weak to retract a large pneumatic tube and support heavy objects.
Also, the retractable force of the spiral springs varies with the length of the inflatable tube (e.g., weak spring force at shorter extension).
Our design contributes to overcoming these challenges for scalable, reliable, and easy-to-fabricate actuation.

\begin{figure}[!h]
\centering
\includegraphics[width=3.4in]{final-figures/system-cad.jpg}
\caption{3D CAD model of the actuator design, including the inflatable tube, the two attached constant force springs, solenoid valve for air supply, servo motor for air release, and bottom plate to fix the inflatable tube.}
~\label{fig:system-cad}
\vspace{-0.6cm}
\end{figure}

\subsection{Design Rationale}
The goal of our system is to {\it provide an accessible prototyping building block for room-scale shape-changing interfaces}. To achieve this goal, we set the following three design requirements:

\subsubsection{Low-cost and Scalable}
Cost and fabrication complexity is essential to lower the barrier of prototyping.
As we discussed, commercially available mechanical actuators are expensive when the system requires a larger size and higher load resistance. Therefore, we considered inflatables for low-cost and scalable actuation methods.

\subsubsection{Robust}
For room-scale applications, the strength and robustness of the actuator is another important factor.
Unlike table-top interfaces, users often interact with room-scale interfaces with their bodies (e.g., leaning against, sitting down, stepping on), thus the actuator must sustain such external force.
We considered inflatables actuators as it can withstand heavy objects, durable for unexpected interactions, and safe for users.

\subsubsection{Compact and Reconfigurable}
Room-scale shape-changing interfaces often require substantial space to install and deploy.
For temporary use or quick prototype, it is impractical to be permanently installed at one location.
Therefore we designed modular, compact, lightweight, and highly customizable units so that the user can quickly pick and place from storage to start prototyping.
% just like placing a tile on the floor.

\subsection{Mechanical Design}
\subsubsection{Plastic Tube and Constant Force Springs}
Here, we describe more detail about design and implementation.
The inflatable element is a 0.15 mm thickness vinyl tube that is 20 cm in diameter when inflated. We cut the tube to an appropriate length and heat-sealed both ends (and cut holes for valves later).  One end of the tube is rolled; the other is fixed to the base plate.
Each constant force spring (Dongguan Yongsheng Metal) has 1.5 m in length, 2 cm in width, and 0.8 kg force.
One end (flat side) of the spring is fixed to the base plate and the other end (rolled side) is fixed to the top end of the tube (Figure~\ref{fig:mechanical-design}).
Once fixed, we tape the spring to the side of the tube.

\begin{figure}[!h]
\centering
\includegraphics[width=3.4in]{final-figures/system-valve.jpg}
\caption{The solenoid valve and the servo motor attached on the base plate (A). The servo motor, rack, and pinion mechanism actuate and move up the silicon tap to change from a closed state (B) to an open state (C) to release internal air.}
~\label{fig:system-valve}
\vspace{-0.6cm}
\end{figure}

\subsubsection{Base Plate and Valves}
The laser-cut base plate (plywood, 3 mm thickness, 22 cm x 22 cm size) has two holes for air supply and release respectively.
The supply hole is fitted with a 1.5 cm diameter solenoid valve (Ebowan Plastic Solenoid Valve DC 12V).
The release hole has a T-shaped silicon tap (Figure~\ref{fig:system-valve}B), which opens and closes (Figure~\ref{fig:system-valve}C) with a 3D printed rack and pinion gear mounted on a servo motor (TowerPro SG90).
This custom silicon tap has a large hole size (4 cm), enabling faster module retraction than common solenoid valves.
Assembly time for each module is approximately 15-30 minutes, and the cost of each actuator is less than 8 USD, including the solenoid valve (3 USD), contact force springs (0.5 USD), servo motor (2 USD), and other material costs.
In total, we fabricated 25 units for our prototype.

\subsubsection{Modular Design}
Each actuator is modular and can connect with the air supply of neighboring actuators. 
Each solenoid air intake valve is connected to a T-fitting. 
Adjacent actuators are pneumatically connected with a silicon tube between the T-fittings (Figure~\ref{fig:system-arrays}). This way, an array of actuators is connected to a shared pressurized supply line.
Air compressors (Yasunaga Air Pump, AP-30P) pressurize the shared line. Each compressor provides up to 12.0kPa of pressure and supplies 30L of air volume per minute. 

\begin{figure}[!h]
\centering
\includegraphics[width=3.4in]{final-figures/system-design.pdf}
\caption{Pneumatic control system for actuator arrays.}
~\label{fig:system-arrays}
\vspace{-0.6cm}
\end{figure}

\subsubsection{Control}
The height of each actuator is controlled by opening and closing a solenoid supply valve and a release tap actuated with a servo motor (Figure~\ref{fig:system-mechanism}).
To control each valve and servo motor, we used two 16 channel 12V relay modules (SainSmart) and 16 channel PWM servo motor drivers (PCA9685) respectively.
The servo motor driver and relay module are controlled from an Arduino Mega Micro-controller.
A Realsense SR300 depth camera mounted on the ceiling (or on a wall for horizontal extension) captures the current height of each actuator.
The software uses this sensor data to control the valves and to achieve the appropriate height.
Our client software written with OpenFrameworks displays the current height and control of each actuator and communicates with the master Arduino through a serial interface.

\begin{figure}[!h]
\centering
\includegraphics[width=3in]{final-figures/system-telescopic.pdf}
\caption{Telescopic structure for a collapsible enclosure. Each square tube is connected with rubber bands (orange) to ensure they do not separate when extended.}
~\label{fig:system-telescopic}
% \vspace{-0.6cm}
\end{figure}

\subsubsection{Telescopic Enclosure}
When positioned vertically, the inflatable actuator has a rounded shape at the top, which is too unstable for stepping, standing or sitting.
Therefore, it is mounted inside a telescoped enclosure to enable the user to sit or step on it.
Each enclosure consists of ten concentric square tubes made of polycarbonate corrugated sheets (3mm thickness), one inside the other (Figure~\ref{fig:system-telescopic}).
We first laser cut the sheets (3mm thickness) and fold them into square tubes, then stack and connect them with Mobilon rubber bands (Nishinbo MB8064TA100G, 6mm thickness, 80mm folding diameter) to ensure they do not separate when extended.
Then, we mount and fix the telescoped enclosure to the base plate with cable ties. 
The top of the enclosure measures 30 cm x 30 cm and, when fully collapsed, 18 cm in height.
We measured the load-bearing capacity of the actuator by placing weights in 2kg increments on top of them. We found that the actuator and the telescopic enclosure can withstand at least 10kg.
With greater load, the telescoped enclosure starts to bend sideways, which made it difficult to accurately measure the maximum load. However, during use, we observed that multiple actuators stacked next to each other resisted bending and can withstand higher loads.


\subsection{Constructive Building Blocks}

\subsubsection{Vertical and Horizontal Orientations}
Due to the relatively compact size and small weight of the modules, various architectural surfaces can be considered for installation, such as placed on the floor or installed sideways from a wall.
% or horizontal surfaces like stairs hung from the ceiling 
% or free-standing pillar

\begin{figure}[!h]
\centering
\includegraphics[width=3.4in]{final-figures/design-space-orientation.jpg}
\caption{Different orientation.}
~\label{fig:design-space-orientation}
\vspace{-0.6cm}
\end{figure}


\subsubsection{Different Sizes and Arrangements}
We also experimented with different sizes, trying footprints of 10 x 10 cm, 20 x 20 cm, and 30 x 30 cm, each of which uses a vinyl tube of 10 cm, 20 cm, and 27 cm in width respectively (Figure~\ref{fig:design-space-size}).
All are made with the same design, but the smaller designs require less force for the spring. We tested with 0.5kgf, 0.9kgf (0.3kgf x 3), 1.5kgf (0.5kgf x 3) for each size respectively.
We did not make the larger size than 30 x 30 cm as we were not able to find an off-the-shelf vinyl tube larger than 27 cm in width.

\begin{figure}[!h]
% \vspace{-0.2cm}
\centering
\includegraphics[width=3.4in]{final-figures/design-space-size.png}
\caption{Different actuator footprints: 10 cm, 20 cm, and 30 cm}
~\label{fig:design-space-size}
\vspace{-0.6cm}
\end{figure}

We observed that a smaller-sized actuator can respond faster, but was less stable under load.
Our final design uses the 30 cm x 30 cm size, as it has a higher load-bearing and a more stable structure, which is better suited for room-scale shape changes. 

% enables interesting applications such as reconfigurable furniture.
% large-scale interaction such as reconfigurable furniture
% a person to sit on a single actuator like a stool, a footprint of 30x30 cm was chosen. 

The actuators can be arranged in a grid, a line, or as individ- ual, loosely arranged units. Figure~\ref{fig:design-space-reconfigurability} depicts a few example configurations, which can also be reconfigured by the person installing them or the end user. An individual actuator can be picked up and moved, which may let the user handle it like a traditional piece of furniture, but could also open up new possibilities for interaction, such as actuators with a motorized base that reconfigures the arrangement according to the current use case.

\begin{figure}[!h]
% \vspace{-0.2cm}
\centering
\includegraphics[width=3.4in]{final-figures/design-space-reconfigurable.png}
\caption{Different actuator arrangements.}
~\label{fig:design-space-reconfigurability}
\vspace{-0.6cm}
\end{figure}











% The direction in which the actuator is usually perpendicular to the base and therefore linked to the installation: vertically upwards when placed on a floor, and horizontally sideways when mounted on a wall. However, there is an interesting space for imagining different configurations, like angled configurations that meet when extended, or a floor actuator that extends sideways to create a wide step.


% To design a building blok for room-scale shape-changing interfaces, we have identified the following three design goals. 
% Given these technical consideration, we set the following three design goals for actuation mechanism for a room-scale shape display.

% \textit{Scalability (Size, Cost, Fabrication Complexity, Number of Elements): }
% We explored a number of designs and prototypes, towards the goal of enabling the easy manufacturing and large footprint for its size.
% It is also important to support different sizes without a significant design changes.

% We designed our actuators, with the goal of achieving a large footprint and high load tolerance, while maintaining the ease fabrication for scalability.
% We explored a number of designs and prototypes, and found that a larger size can provide higher stability.
% We hypothesize the pneumatic actuation is suitable for this design requirement as it allows the system to be low-cost, easy to fabrication, lightweight, safe, and maintain a high power-to-weight ratio.
% Pneumatic actuators are also durable, and do not require power to maintain the state, which contributes to the power consumption.
% A simple, liehgtweight, and compact unit allows the user to easily install and customize based on their needs, and suitable for storage and portability.
% \subsubsection{Pneumatic Control System}
% Each individual actuator is modular and can be connected with the neighboring actuators. 
% At the end of the solenoid air intake valve of each actuator, it is connected to a T-shaped plumbing joint. 
% Adjacent actuators are pneumatically connected through a silicon tube between the T-shape joints. This way, an array of actuators is connected to a shared pressurized line.



% Likewise, the extension of the actuator can be modified by changing the length of the internal pneumatic tube and spring. When placed inside a collapsing enclosure, our actuator extends from a collapsed size of 15 cm to an extended size of 100 cm, due to the overwrap between each telescopic box.
% Here, we show three different sizes based on the diameter of the pneumatic tube.
% Smaller size requires less force. In this prototype, we used one 1.5m 0.8kgf or three 1.5m 0.5kgf springs
% Extension ratio of each actuator depends on the length of contact force spring. 
% We used two 1.5m 0.8kgf or three 1.5m 0.5kgf springs.
% We report technical evaluation in two aspects: load bearing and speed of expansion and contraction. 
% The module size refers to the footprint of the actuator and the overall dimensions when retracted and extended. As the pneumatic actuation tubes can be modified for different diameters and length, fabricating actuators with different sizes is straightforward. 



% \begin{figure}[!h]
% \centering
% \includegraphics[width=3.2in]{anonymous-figure/applications-chair.png}
% \caption{Dynamic furniture. \tool{} creates a chair as a person approaches. These objects later disappear once no longer needed.}
% ~\label{fig:applications-chair}
% \end{figure}



==> TEI 2020 - LiftTiles_ Constructive Building Blocks for Prototyping Room-scale Shape-changing Interfaces/7-applications.tex <==
\section{Prototyping Applications}
To gauge how well \tool{} is suited to our goal of supporting rapid prototyping and user testing, we built several different example applications.
These were inspired by existing shape-changing interfaces, which we categorized into the following high-level application spaces: 1) {\it adaption:} adapting to users' needs and context~\cite{yao2013pneui, nakagaki2015lineform, roudaut2013morphees, gomes2013morephone, follmer2013inForm, gross2012architectural}, 2) {\it display:} communicating with the user by displaying information or data~\cite{follmer2013inForm, taher2015exploring, suzuki2018dynablock, goulthorpe2001aegis}, and 3) {\it haptics}: providing haptic feedback synchronized with visual information~\cite{siu2018shapeShift, teng2018pupop, delazio2018force, iwata2001project}.
Figure~\ref{fig:applications-sketch} depicts a concept sketch of applications resulting from an initial brainstorming. The following example applications were all chosen to leverage large-scale shape change and built in less than a day.

\subsubsection*{Adaptive Floor Furniture}
The first application is a reconfigurable floor that creates adaptive furniture, inspired by an adaptive dynamic table (e.g., TRANSFORM~\cite{vink2015transform}) and dynamic physical affordances (e.g., inFORM~\cite{follmer2013inForm}).
We created a shape-changing floor by arranging 25 modules in a 5 x 5 grid. Each unit is individually actuated to provide a chair, a table, and a bed (Figure~\ref{fig:cover}).

\subsubsection*{Shape-changing Wall}
By leveraging the block's compact form factor, we also prototyped a horizontal shape-changing wall to adapt to user needs and display information.
The wall becomes a space separator to make a temporary meeting space, while it can also act as public signage by displaying an arrow shape to guide a passer-by.
% By stacking multiple horizontal displays along a wall, they can render more expressive information, such as forming a pictograph through negative space.

\begin{figure}[!h]
\centering
\includegraphics[width=3.4in]{final-figures/applications-wall.jpg}
\caption{Adaptive space separation. The wall creates a temporary meeting space by separating the space, and changes shape to display an arrow.}
~\label{fig:applications-separation}
\vspace{-0.6cm}
\end{figure}

\subsubsection*{Deployable Pop-Up Structure}
As the actuators are compact compared to traditional furniture and walls, they can be deployed in temporary use cases such as festivals, trade shows, concerts, and disaster relief.
In these applications, the actuators are shipped in a compact box and laid out in an empty room, similar to tiles.
After connecting them to a compressor and control computer, the operator selects a use case and the blocks render a layout of chairs, beds, tables, and partitions.
% This arrangement could be pre-programmed or it could be defined by the operator on-site by specifying what shapes to extrude. After the event, the actuators contract into compact tiles and can be stored for future use.

\begin{figure}[!h]
\centering
\includegraphics[width=3.4in]{final-figures/system-modular.png}
\caption{Modular design to construct different geometries.}
~\label{fig:system-modular}
\vspace{-0.6cm}
\end{figure}

\subsubsection*{Landscape Haptics for VR}
While hand-sized shape displays have rendered haptic sensations for VR~\cite{siu2018shapeShift}), we propose to render furniture-size props, walls, and game elements that users can feel through walking and touching while experiencing immersive VR scenes.
\changes{Similar to the applications proposed by HapticTurk~\cite{cheng2014haptic}, TurkDeck~\cite{cheng2015turkdeck}, and TilePop~\cite{teng2019tilepop}, In this application, the haptics increases the feeling of presence in games by providing room-scale dynamic haptic feedback.}
Also, this can aid the design process by rendering full-scale object mock-ups of large objects like a car.

\begin{figure}[!h]
\centering
\includegraphics[width=3.4in]{final-figures/applications-haptics.png}
\caption{Room-scale dynamic haptics for VR.}
~\label{fig:applications-haptics}
% \vspace{-0.6cm}
\end{figure}

\subsubsection*{Dynamic Data Physicalization}
Inspired by related work in dynamic data physicalization~\cite{Jansen:2015:OCD:2702123.2702180, taher2015exploring}, this exhibit enables for a tangible exploration of data.
On the floor, a timeline of the last 2,000 years is shown, and visitors move an actuator module along the timeline. The actuator dynamically extends or retracts to represent the average body height of a person of the same age at the given period. For example, a 10 years old girl can see and feel how children 100 years ago were of a different average height.
% We made this for a data discovery room in a science museum.


\begin{figure*}[!h]
\centering
\includegraphics[width=\textwidth]{final-figures/applications-sketch.pdf}
\caption{Concept sketch of application scenarios, inspired by existing shape-changing interface research.
Orange part represents each LiftTile module.
(A) Wall-based display for wayfinding guidance.
(B) The room-scale shape display that becomes a chair, a table, or a bed.
(C) Large-scale haptics for virtual and augmented reality.
(D) Pick up and place for deployable pop-up structure.
}
~\label{fig:applications-sketch}
\vspace{-0.6cm}
\end{figure*}


% \subsubsection{Full-scale Design Mock-up}
% Similarly, in domains like car design or interior design, it is important to see the object as a full-scale mock-up during their design process.
% To aid this design process, the floor-based shape display can provide an instant real-scale object mock-up, so that they can see, touch, and modify the car design.

% For example, despite the dominance of CAD tools, car designers still create full-scale clay models for design modifications and reviews.

% For the second process, we were particularly interested in the insights from their professional point of view, and to identify what kind of prototypes they would want to use the system for. We then asked the participants open-ended questions about possible use cases and practicality. Each interview took approximately 60 minutes.




% This approach could also be combined with the idea of human actuation~\cite{cheng2015turkdeck}, where human actors place objects to provide large-scale force feedback for a user in VR.
% For example, when the actors place the module at the instructed location, the module can automatically change its height to create a haptic proxy object like a table or a wall.
% Thus, by leveraging the reconfigurability and instructions for human volunteers that continuously rearrange modules in an open area, the system can provide room-scale haptic sensations with a much smaller number of modules.



% such as bar charts, 3D map data, and body-scale data sculptures.
% For example, Figure~\ref{fig:applications-display} illustrates a \tool{} pillar rendering the population pyramid of a country.
% Such public large-scale data physicalizations can engage people and attract attention. In addition, \tool{} can provide interactive spatial data physicalizations.



% When a user asks for directions, the pillar transforms to render an arrow shape pointing towards the target location


% In addition to adapting for functional use as furniture, \tool{} can also communicate with the user by displaying information through shapes. For instance, \tool{} acts as a public signage display by extending an array of horizontal actuators from a pillar. When a user asks for directions, the pillar transforms to render an arrow shape pointing towards the target location (see Figure~\ref{fig:dynaroom-prototype}).
% By stacking multiple horizontal displays along a wall, they can render more expressive information and animation. When extending all of the actuators, these display sections cover the wall, when retracting them selectively, they can form a pictograph through negative space.

% \subsubsection{Deployable Pop-Up Structure}
% As the \tool{} actuators are compact compared to traditional furniture and walls, they can be deployed in temporary use cases like festivals, trade show, concert stages, and disaster relief quarters.
% In this application, the actuators are shipped in a compact box and laid out inside an empty room, similar to tiles.
% After connecting them to a compressor and control computer, the operator selects a use case and they render a layout of chairs, beds, tables, and partitions. This arrangement could be pre-programmed or it could be defined by the operator on site by specifying what shapes to extrude. After the event, the actuators contract into compact tiles and can be stored for future use.


% An interesting question in this application is how the room interacts with users and objects while transforming between the different configurations. By sensing the persons presence, the room would avoid rendering elements where they currently stand, or even create barriers like a safety fence around a transforming section.
% Also, \tool{} could be combined with custom built static objects. As an example, the system may render the legs of tables and chairs, onto which a lightweight tabletop and seating cushions are placed. These static objects could be used to issue commands to the system: When a user holds a seating cushion at a certain position and issues a command, \tool{} renders legs at that specific location and height, and when removing the cushion, these legs automatically disappear.

% Besides the user picking up and moving objects in the room, \tool{} could also transform it's surface to slide or tumble objects into their desired position, similar to how prior work moves and assembles objects on smaller shape displays \cite{schoessler2015kinetic}.



% These deployable structures can also provide on-demand assistance.
% For example, \tool{} could make a stool, so that children can stand on the module to reach an object at the kitchen, or a book in a bookshelf.
% Alternatively, these deployable structures can create an on-demand accessibility assistant.
% For example, by placing a plate on multiple \tool{} modules, it can create a ramp for wheel-chair users.


% \subsubsection{Dynamic Data Physicalization}
% \tool{} can render data physicalizations, such as bar charts, 3D map data, and body-scale data sculptures.
% For example, Figure~\ref{fig:applications-display} illustrates a \tool{} pillar rendering the population pyramid of a country.
% Such public large-scale data physicalizations can engage people and attract attention. In addition, \tool{} can provide interactive spatial data physicalizations.
% An example of such an application would be a data discovery room in a science museum. A ceiling-mounted projector projects a timeline of the last 2,000 years onto the floor.
% Children pick up a \tool{} module and place it on a time period, then the actuator extends to represent the average body height of the same age at the given time period.
% This way, 10 years old girl can see and feel how children 100 years ago were of a different average height.
% Such body-scale data physicalizations encourage spatial thinking and discovery to relate to data in meaningful new ways~\cite{Jansen:2015:OCD:2702123.2702180}.

% \begin{figure}[!h]
% \centering
% \includegraphics[width=3.2in]{figures/applications-display.png}
% \caption{Displaying a bar graph that represents a population pyramid.}
% ~\label{fig:applications-display}
% \vspace{-0.6cm}
% \end{figure}

% \subsection{Haptics}
% \subsubsection{Haptics for VR}
% \tool{} can improve virtual or augmented reality experiences by rendering room-scale haptic objects.
% For example, when the user puts on a headset and starts a game, the room can transform its shape to synchronize the physical landscape to the virtual one.
% The actuators can mimic furniture, walls, and bumps so that the user can feel the haptic sensation through walking and touching.
% This approach could also be combined with the idea of human actuation~\cite{cheng2015turkdeck}, where human actors place objects to provide large-scale force feedback for a user in VR.
% For example, when the actors place the module at the instructed location, the module can automatically change its height to create a haptic proxy object like a table or a wall.
% Thus, by leveraging the reconfigurability and instructions for human volunteers that continuously rearrange modules in an open area, the system can provide room-scale haptic sensations with a much smaller number of modules.

% \begin{figure}[!h]
% \centering
% \includegraphics[width=3.2in]{figures/applications-haptics.png}
% \caption{Room-scale dynamic haptics for VR.}
% ~\label{fig:applications-haptics}
% \vspace{-0.6cm}
% \end{figure}

% \subsubsection{Full-scale Design Mock-up for AR}
% In domains like car design or interior design, it is important to see the object as a full-scale mock-up during their design process.
% For example, despite the dominance of CAD tools, car designers still create full-scale clay models for design modifications and reviews.
% To aid this design process, \tool{} can provide an instant real-scale object mock-up, so that they can see, touch, and modify the car design. By combining \tool{} with augmented reality headsets, realistic renderings can be overlaid on top of the physical mockup (see Figure~\ref{fig:cover}).



% Moreover, our modular and reconfigurable design allows researchers and designers to quickly construct different geometries and to explore various applications.
% This paper contributes to the design and implementation of highly extendable inflatable actuators, and demonstrates a range of scenarios that can leverage this modular building block.











% In a science museum
% - bar chart
% - google maps
% - map data
% - theatrical performance

% These displayed pictographs or silhouettes can also animate by controlling the length of each pin.
% The shape display can also provide a dynamic data physicalization.
% For example, at the working space, the horizontal shape display can visualize the working time within a week by using seven actuated pins.


% In collaboration with the occupant the room could provide instructions on where to place objects or temporary surfaces for storing them during the transition.
% This combination of static and dynamic elements can provide the desired look and feel for the surfaces that the user touches. But at the same time, the static furniture elements are more compact and lightweight and easier to move and store.

%  Alternatively, a wheeled robot could move the object in and out of place.



% To allow these designers to see, touch, and modify the current design at real-scale, the shape display can provide a real-scale object mock-up.
% By combining with the augmented reality headsets, the user can not only see the design, but also touch and modify them through tangible interactions.

% each module can provide more dynamic haptic environment by combining the locomotion such as using movable robots~\cite{iwata2005circulafloor} or human actuation.
% For example, by using a human to move each module based on the
% it can provide more various haptic sensation, while reducing the manual elements.
% For example, when a ``turker'' places the module to the different location, then the module can automatically change its height to create a wall.

% Thus, the turkers can only move these modules one by one,

% \tool{}'s actuators can render surfaces and spaces to augment a virtual reality experience. By combining \tool{} with VR techniques like redirected walking, a small space can create a seemingly expansive, ever changing game area.

% Combining with human actuation

% For example, similar to, the dynamic room can make a temporal wall for VR games.

% By actuating an existing object, it can also make an instant theme park.
% For example, in the boat game, the user makes the boat with a cardboard, then the shape display makes the dynamic wave, which makes an experience as if the user actually cruise down the river.



% can provide a realistic rendering for these designs, but it lacks the physical sensation.
% \tool{} can also provide an instant preview of the large-scale object.
% A user can check how big a furniture to see if it fits a room, the shape displaying wall can show an actual size of the furniture.
% A car designer renders the current car design from the cad to see its two-dimensional or even three-dimensional silhouette in the actual size.



%  through showing a pictograph
% when asking which way to go, then arrow shape appears.
% \tool{} can morph not only for functional purposes, but also to display information or attract attention. Figure  depicts a scenario where a dynamically rendered arrow shape guides the user into the right direction in a public space.



% These objects can be appe be disappeared once the user no longer needs it.
% extend a desk and create a temporal chair for the additional participants.
% Similarly, dynamic architecture can also provide an adaptive space separation, but in more dynamic and programmable manner.
% If a child needs a footrest under her chair in the dining room, then it can provide a situated footrest. And the height of the footrest can be changed as she grows.
% One example is an adaptive object appearance.
% In traditional architectures, we have seen many adaptive architectures through manual reconfiguration.
% For example, traditional Japanese style architectures utilize slidable partition called Shoji or Fusuma, to allow a user to change the space separation based on the user's room requirements.
% For example, in the public working space, one person is working on a table.
% When another person approaches the table to work on at the next, the dynamic wall can create a temporal partition to make a space more private.






% \begin{figure}[!h]
% \centering
% \includegraphics[width=3in]{draft-figure/system-multiple.jpg}
% \caption{Extension.}
% ~\label{fig:design-fabrication}
% \end{figure}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=3in]{draft-figure/system-fabrication.JPG}
% \caption{Fabrication process.}
% ~\label{fig:design-fabrication}
% \end{figure}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=3in]{draft-figure/system-extend.png}
% \caption{Extension.}
% ~\label{fig:design-fabrication}
% \end{figure}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=3in]{draft-figure/system-size.png}
% \caption{Different sizes with the same design.}
% ~\label{fig:design-fabrication}
% \end{figure}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=3in]{draft-figure/system-weight.png}
% \caption{Technical evaluation for weight.}
% ~\label{fig:design-fabrication}
% \end{figure}



==> TEI 2020 - LiftTiles_ Constructive Building Blocks for Prototyping Room-scale Shape-changing Interfaces/8-limitations.tex <==

% \section{Discussion}

\section{Limitations and Future Work}
During the process of prototyping example applications, we confirmed that the modularity and simplicity of \tool{} are well-suited for rapid prototyping, but we also discovered a number of limitations that we plan to address in future work. 

\subsubsection*{Load Tolerance}
Although the pneumatic actuator can withstand heavier load than 10 kg, our outer enclosure is insufficiently stable and robust, as discussed in the system section (see Telescopic Enclosure).
We added the fabricated enclosure to stabilize the top, but as it is manually fabricated out of plastic cardboard, the structure becomes unstable when loaded with heavy objects.
\changes{A user can sit on a single actuator, but has to actively maintain balance while sitting, which is not ideal even for prototyping scenarios. }
A more precisely manufactured telescoping structure would greatly increase the load tolerance.
\changes{An alternative possible solution would be to use a bi-stable or mono-stable extendable structure such as tuneable mechanical truss~\cite{yasuda2017origami}, origami-based enclosure~\cite{zhai2018origami}, and {\it coilable} masts~\cite{joosten2007preliminary}, inspired by deployable structures explored for space applications~\cite{jensen2001arm} (e.g., deployable antennas and masts.)
Finally, combining multiple reel-based tubes inside each block can make them more stable. This design also allows the larger blocks than 30 cm. 
One potential challenge is that each tube may inflate at a different speed even if air comes from the same supply hole, but this can be addressed by using pressure sensor or height sensor to control the amount of air to be supplied.
We will also investigate this as future work}


\subsubsection*{Speed of Transformation}
One current limitation is the slow speed of transformation. In our current setting, \changes{it takes 16 seconds to fully extend a module and 4 seconds to fully retract it}.
There are some potential solutions, such as using a stronger air compressor and larger valves, but the speed of transformation of large inflatables is generally slower than electromechanical actuation. 
It is therefore difficult to prototype applications that require fast shape transformation, such as VR games. Interactions similar to the ones proposed in related work like TurkDeck~\cite{cheng2015turkdeck} and TilePop~\cite{teng2019tilepop} can be utilized to maintain a sense of presence for the user even with slow transformations.

\subsubsection*{Lack of Interactivity}
This paper we focused primarily on the {\it output} of shape-changing interfaces and less on sensing user input.
Adding input sensing modalities such as embedded touch sensing would greatly increase the interactive capabilities.
\changes{For future work, incorporating the sensing methods proposed by~\cite{swaminathan2019input} (e.g., acoustic, capacitive, and pressure sensing) should be explored to improve the interactivity of the current prototype.}
We are also interested in using a dynamic appearance (e.g., color changing with LEDs) to provide different affordances.

\subsubsection*{Different Height Tracking}
IR photo reflectors or pressure sensors could replace the external camera for a more robust internal height sensing.
We observe that sometimes two similar tubes extend at a different rate, although inflating from the same pump.
More precise and embedded sensing can achieve more consistent speed and control.

\subsubsection*{Distributed Control}
Currently, we are controlling each module through a central Arduino board, which requires a cumbersome electric connection with wires. We are interested in improving the modularity of each unit by using a Wifi chip module (e.g., ESP8266) to control wireless communication. This would also allow easy mapping between modules and the software interface (currently, we need to manually map at the beginning.) 
We are also interested in adding mobility in each unit to allow for autonomous and distributed room-scale shape-changing interfaces. 

\subsubsection*{User Evaluation}
All our prototypes are created by us, and we have not formally evaluated the system with a user study. As a next step, we plan a workshop with researchers and designers (e.g., interior designers and architects) to explore and prototype, similar to ~\cite{hardy2015shapeclip}.
We expect a formal evaluation to provide insights into how this tool supports design ideation.
% In the future, we are interested in deploying this prototype and observe how users interact with it, in a similar spirit to the observational study of large-scale shape-changing interfaces~\cite{gronvall2014causing}.


% We anticipate another actuation methods may be suitable for fast and highly dynamic shape transformation. 
% Most of the application scenarios we explored may not require the fast speed of transformation, but for some scenarios such as dynamic haptics for VR, the current configuration may not be fast enough.
% Multiple stronger air compressors can solve these issues, but the noise of the compressor will be another problem. 

% \subsubsection{Modular and Mobile Shape Displays}
% Currently, each module needs to be connected to the central computer. 
% Each control signal and power supply came from the central microcontroller and power sources.
% We are interested in having each actuator can have its own microcontroller and power supply, so that it can increase the modularity and flexibility.
% Moreover, we are interested in adding the locomotion functionality for each module, inspired by \cite{iwata2005circulafloor}.
% The mobility allows an autonomous and distributed large-scale shape display which can deploy, extend, and store by themselves.
% We envision these modular and locomotive actuation units can further transform our physical space to dynamic and interactive environments for Human-Architecture Interaction.


% which limits the interactivity of the current prototype.
% Also, as we saw in the expert review, there are many interactive applications that can be connected with data (e.g., rendering a 3D map).
% While we did not prototype these features, we think these color change can also provide some affordances.











==> TEI 2020 - LiftTiles_ Constructive Building Blocks for Prototyping Room-scale Shape-changing Interfaces/9-conclusion.tex <==


\section{Conclusion}
This paper introduces constructive building blocks for prototyping room-scale shape-changing interfaces.
To this end, we designed a modular inflatable actuator that is highly extendable (from 15cm to 150cm), low-cost (8 USD), lightweight (10 kg), compact (15 cm), and strong (e.g., can support 10 kg weight) making it well-suited for prototyping room-scale shape transformations.
Moreover, our modular and reconfigurable design allows researchers and designers to quickly construct different geometries and to investigate various applications.
In this paper, we contributed to the design and implementation of highly extendable inflatable actuators, and demonstrates a range of scenarios that can leverage this modular building block.
We plan to evaluate the potential of our system by inviting designers to use our blocks in their own designs and see whether and/or how our building blocks enhances their ideation process. 


% design space for room-scale shape displays, implement a prototype system and ideate applications with three domain experts. Based on their feedback, we propose a number of example applications and envision scenarios for reconfigurable architectural spaces, temporary deployable pop-up structures, and haptic feedback for VR. 

% \tool{}, a modular and reconfigurable room-scale shape display. To achieve actuation of furniture scale objects, we design and implement a retractable inflatable actuator, which enables a compact, lightweight, modular structure. We propose a design space for room-scale shape displays, implement a prototype system and ideate applications with three domain experts. Based on their feedback, we propose a number of example applications and envision scenarios for reconfigurable architectural spaces, temporary deployable pop-up structures, and haptic feedback for VR. 

% In this paper, we introduced Dynaroom, a system to explore room-scale Human-Architecture Interaction. Based on an array of low-cost, light-weight, and high load-bearing pneumatic linear actuators, we demonstrate how floors and walls can turn into dynamic interactive surfaces. These room-scale shape displays render partitions and furniture on demand, display information physically and provide dynamic haptic feedback. We envision applications scenarios for reconfigurable architectural spaces, temporary deployable pop-up structures, and Virtual Reality. 

==> TEI 2020 - LiftTiles_ Constructive Building Blocks for Prototyping Room-scale Shape-changing Interfaces/acknowledgements.tex <==
\section{Acknowledgements}
We thank Shohei Takei for helpful suggestions.
This research was supported by the JST ERATO Grant Number JPMJER1501 and the Nakajima Foundation.

==> TEI 2020 - LiftTiles_ Constructive Building Blocks for Prototyping Room-scale Shape-changing Interfaces/changes.tex <==
Summary of Changes

Major points
-  cited the previous submission in UIST 2019 adjunct and describe the difference in terms of the design rationale, technical description, and limitations of the system in detail.
-  discussed the difference to TileTop
-  cited missing references pointed by R1 and R3 (e.g., Swaminathan et al, TrussFormer, TrussFab, Protopiper, HapticTurk)
-  added a thorough discussion of limitations and discuss the possible solution for future improvements

Minor points
-  added the contraction time
-  fixed reference 7 and 16
-  removed Figure 1-E as it presents the same configuration twice
-  added annotation for figure 5


==> changes.tex <==
Summary of Changes

Major points
-  cited the previous submission in UIST 2019 adjunct and describe the difference in terms of the design rationale, technical description, and limitations of the system in detail.
-  discussed the difference to TileTop
-  cited missing references pointed by R1 and R3 (e.g., Swaminathan et al, TrussFormer, TrussFab, Protopiper, HapticTurk)
-  added a thorough discussion of limitations and discuss the possible solution for future improvements

Minor points
-  added the contraction time
-  fixed reference 7 and 16
-  removed Figure 1-E as it presents the same configuration twice
-  added annotation for figure 5

